On the Importance of Opponent Modeling in Auction Markets

The dynamics of financial markets are driven by the interactions between participants, as well as the trading mechanisms and regulatory frameworks that govern these interactions. Decision-makers would rather not ignore the impact of other participants on these dynamics and should employ tools and models that take this into account. To this end, we demonstrate the efficacy of applying opponent-modeling in a number of simulated market settings. While our simulations are simplified representations of actual market dynamics, they provide an idealized "playground" in which our techniques can be demonstrated and tested. We present this work with the aim that our techniques could be refined and, with some effort, scaled up to the full complexity of real-world market scenarios. We hope that the results presented encourage practitioners to adopt opponent-modeling methods and apply them online systems, in order to enable not only reactive but also proactive decisions to be made.

==> fig/single_auction/index.tex <==
\begin{figure}[!h]
\centering
\begin{subfigure}[b]{0.5\linewidth}
  \begin{subfigure}[l]{0.32\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/replicator_dynamics/FP_IPG__quiver.pdf}
  \end{subfigure}
  \begin{subfigure}[l]{0.32\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/replicator_dynamics/FP_NEU__quiver.pdf}
  \end{subfigure}
  \begin{subfigure}[l]{0.32\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/replicator_dynamics/IPG_NEU__quiver.pdf}
  \end{subfigure}
  
  \begin{subfigure}[l]{0.32\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/replicator_dynamics/FP_IPG__streamplot.pdf}
  \end{subfigure}
  \begin{subfigure}[c]{0.32\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/replicator_dynamics/FP_NEU__streamplot.pdf}
  \end{subfigure}
  \begin{subfigure}[r]{0.32\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/replicator_dynamics/IPG_NEU__streamplot.pdf}
  \end{subfigure}
\caption{Multi-population replicator dynamics.}
\end{subfigure}
\begin{subfigure}[b]{0.36\linewidth}
    \includegraphics[width=\linewidth]{fig/single_auction/empirical_payoff_table.pdf}
\caption{Empirical payoff table.}
\end{subfigure}
\caption{Empirical results for bidding strategies: Fictitious Play (FP), Implicit Policy Gradient (IPG) and Nash Equilibrium for anonymous single auction with Uniform private evaluations (NEU). FP is the dominant stable equilibrium over both IPG and NEU, while the adaptive IPG dominates over the static NEU. In figure (a) the $x$-axis is the probability of player 1 following strategy $i$, termed $p^{(1)}(i)$, and the $y$-axis for player 2 accordingly. The visualizations are made using the open-source tool \texttt{OpenSpiel}~\citep{lanctot2019openspiel}.}
\label{fig:single-side-auction}
\end{figure}
